Humanoid Self-Collision Avoidance Using Whole-Body Control with Control Barrier Functions

This work combines control barrier functions (CBFs) with a whole-body controller to enable self-collision avoidance for the MIT Humanoid. Existing reactive controllers for self-collision avoidance cannot guarantee collision-free trajectories as they do not leverage the robot's full dynamics, thus compromising kinematic feasibility. In comparison, the proposed CBF-WBC controller can reason about the robot's underactuated dynamics in real-time to guarantee collision-free motions. The effectiveness of this approach is validated in simulation. First, a simple hand-reaching experiment shows that the CBF-WBC enables the robot's hand to deviate from an infeasible reference trajectory to avoid self-collisions. Second, the CBF-WBC is combined with a linear model predictive controller (LMPC) designed for dynamic locomotion, and the CBF-WBC is used to track the LMPC predictions. Walking experiments show that adding CBFs avoids leg self-collisions when the footstep location or swing trajectory provided by the high-level planner are infeasible for the real robot, and generates feasible arm motions that improve disturbance recovery.

==> drafts/old_abstract.tex <==
This work combines control barrier functions (CBFs) with a whole-body controller to enable joint limit and self-collision avoidance for the MIT Humanoid. 
While trajectory optimization can only satisfy these requirements offline, existing online controllers for self-collision avoidance cannot guarantee kinematic feasibility because they do not leverage the robot's full dynamics.
In contrast, the proposed controller, the CBF-WBC, can reason about the robot's underactuated dynamics in real time to guarantee future kinematic feasibility while satisfying contact constraints.
We validate the effectiveness of this approach in simulation. First, using a simple hand reaching experiment, we show that the CBFs give the robot the ability to deviate from a infeasible reference trajectory to avoid self-collisions. Second, we combine the CBF-WBC with a linear model predictive controller (LMPC) based on a single-rigid body model designed for dynamic locomotion. We found that combining CBFs with a centroidal momentum task generates feasible, unauthored arm motions that can assist humanoid locomotion and disturbance recovery. Finally, the CBFs allow to avoid leg self-collisions when the footstep location predicted by the LMPC is infeasible for the real robot.
